NGC6240: extended CO structures and their association with shocked gas

We present deep CO observations of NGC6240 performed with the IRAM Plateau de Bure Interferometer (PdBI). NGC6240 is the prototypical example of a major galaxy merger in progress, caught at an early stage, with an extended, strongly-disturbed butterfly-like morphology and the presence of a heavily obscured active nucleus in the core of each progenitor galaxy. The CO line shows a skewed profile with very broad and asymmetric wings detected out to velocities of -600 km/s and +800 km/s with respect to the systemic velocity. The PdBI maps reveal the existence of two prominent structures of blueshifted CO emission. One extends eastward, i.e. approximately perpendicular to the line connecting the galactic nuclei, over scales of ~7 kpc and shows velocities up to -400 km/s. The other extends southwestward out to ~7 kpc from the nuclear region, and has a velocity of -100 km/s with respect to the systemic one. Interestingly, redshifted emission with velocities 400 to 800 km/s is detected around the two nuclei, extending in the east-west direction, and partly overlapping with the eastern blue-shifted structure, although tracing a more compact region of size ~1.7 kpc. The overlap between the southwestern CO blob and the dust lanes seen in HST images, which are interpreted as tidal tails, indicates that the molecular gas is deeply affected by galaxy interactions. The eastern blueshifted CO emission is co-spatial with an Halpha filament that is associated with strong H2 and soft X-ray emission. The analysis of Chandra X-ray data provides strong evidence for shocked gas at the position of the Halpha emission. Its association with outflowing molecular gas supports a scenario where the molecular gas is compressed into a shock wave that propagates eastward from the nuclei. If this is an outflow, the AGN are likely the driving force.

==> PaxHeader/n6240_05nov_arxiv.tex <==
18 gid=2048330233
17 uid=346135205
20 ctime=1352112522
20 atime=1352113117
38 LIBARCHIVE.creationtime=1352112217
24 SCHILY.dev=234881026
23 SCHILY.ino=24936019
18 SCHILY.nlink=1

